A Type System for proving Depth Boundedness in the pi-calculus

The depth-bounded fragment of the pi-calculus is an expressive class of systems enjoying decidability of some important verification problems. Unfortunately membership of the fragment is undecidable. We propose a novel type system, parameterised over a finite forest, that formalises name usage by pi-terms in a manner that respects the forest. Type checking is decidable and type inference is computable; furthermore typable pi-terms are guaranteed to be depth bounded. The second contribution of the paper is a proof of equivalence between the semantics of typable terms and nested data class memory automata, a class of automata over data words. We believe this connection can help to establish new links between the rich theory of infinite-alphabet automata and nominal calculi.

==> proofs/subj-red-sketch.tex <==
From $P\redto Q$ we know that
$P \congr \new W.(S \parallel R \parallel C)$,
$S \congr \out a<b>.\new Y_s.(S'+M_s)$,
$R \congr \inp a(x).\new Y_r.(R'+M_r)$,
$Q \congr \new W Y'_s Y'_r.
  (S'\sigma_s \parallel R'\subst{x->b}\:\sigma_r \parallel C)$
where $\sigma_k \is \subst{y->y'}_{y\in Y_k}$,
and $Y'_k \is \Set{y'|y\in Y_k}$ are fresh names,
for $k\in\set{s,r}$.
Then it is easy to verify that
the typing proof of $P$ can be easily adapted to be one for $Q$;
the non trivial step is showing that
the premises involving $R'\subst{x->b}$ are true;
for this we can use Lemma~\ref{lemma:subst}.


==> style/layout.tex <==
\usepackage{fixltx2e}
\let\labelindent\relax
\usepackage[inline]{enumitem}
\setlist[itemize]{label=-}

\newlist{defenum}{enumerate}{2}
\setlist[defenum]{
  label=\small(\roman*),
  ref=\thedefinition.\roman*,
  labelwidth=3pt
}

\newlist{asparaenum}{enumerate}{3}
\setlist[asparaenum]{label=(\roman*), align=left, leftmargin=0pt, labelindent=!, listparindent=\parindent, labelwidth=0pt, itemindent=!}

\newlist{inparaenum}{enumerate*}{3}
\setlist[inparaenum]{label=\alph*)}

\newlist{asparaitem}{enumerate}{3}
\setlist[asparaitem]{label=-, align=left, leftmargin=0pt, labelindent=!, listparindent=\parindent, labelwidth=0pt, itemindent=!}

% \usepackage{booktabs}
% \usepackage{multirow}

\RequirePackage{xcolor}
\usepackage{hyperref}
\hypersetup{final}
\hypersetup{%
    % bookmarks,
    bookmarksopen,
    % bookmarksnumbered,
    colorlinks,
    linkcolor=blue,
    citecolor=brown,
    % backref,
    urlcolor=blue,
    pdfstartview=FitH}
% \urlstyle{same}  % don't use monospace font for urls

%%%% Activate page numbers for conference mode
\makeatletter
\ifCLASSOPTIONconference
  \def\@oddfoot{\hbox{}\hfil \scriptsize \thepage}
  \def\@evenfoot{\hbox{}\hfil \scriptsize \thepage}
\fi
\makeatother
\def\IEEEproofindentspace{0pt}

